Reverberant sound field equalisation for an enhanced stereo playback experience

The topic of room equalisation has been at the forefront of research and product development for many years, with the aim of increasing the playback quality of loudspeakers in reverberant rooms. Traditional room equalisation systems comprise of a number of filters that when applied to the primary loudspeakers, additional room colouration is compensated for. This publication introduces a novel equalisation technique where gammatone filter band energy is added to the reverberant sound field via two surround loudspeakers, leaving the direct sound from the primary loudspeakers unaltered, but the sum of direct and reverberant energy is equalised at the listening position. Unlike traditional systems, this method allows the target function of the direct sound to differ from the reverberant sound field. The proposed method is motivated by the different roles direct and reverberant sound components play in humans perception of sound. Along with introducing the proposed method, results from a subjective listening test are presented, demonstrating the preference towards the proposed technique when compared to a traditional room equalisation technique and stereo playback.

==> Stereo.tex <==
% Created by tikzDevice version 0.12.4 on 2023-03-28 13:55:02
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (1084.05,597.46);
\begin{scope}
\path[clip] ( 49.20, 61.20) rectangle (1058.85,548.26);
\definecolor{fillColor}{RGB}{211,211,211}

\path[fill=fillColor] (109.97,135.61) --
	(296.94,135.61) --
	(296.94,304.73) --
	(109.97,304.73) --
	cycle;
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 1.2pt,line join=round] (109.97,220.17) -- (296.94,220.17);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (203.45,107.43) -- (203.45,135.61);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (203.45,361.10) -- (203.45,304.73);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (156.71,107.43) -- (250.20,107.43);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (156.71,361.10) -- (250.20,361.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (109.97,135.61) --
	(296.94,135.61) --
	(296.94,304.73) --
	(109.97,304.73) --
	cycle;

\path[fill=fillColor] (343.68,135.61) --
	(530.65,135.61) --
	(530.65,220.17) --
	(343.68,220.17) --
	cycle;

\path[draw=drawColor,line width= 1.2pt,line join=round] (343.68,149.70) -- (530.65,149.70);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (437.17, 79.24) -- (437.17,135.61);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (437.17,304.73) -- (437.17,220.17);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (390.42, 79.24) -- (483.91, 79.24);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (390.42,304.73) -- (483.91,304.73);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (343.68,135.61) --
	(530.65,135.61) --
	(530.65,220.17) --
	(343.68,220.17) --
	cycle;

\path[fill=fillColor] (577.40,220.17) --
	(764.37,220.17) --
	(764.37,332.91) --
	(577.40,332.91) --
	cycle;

\path[draw=drawColor,line width= 1.2pt,line join=round] (577.40,276.54) -- (764.37,276.54);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (670.88,163.80) -- (670.88,220.17);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (670.88,417.47) -- (670.88,332.91);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (624.14,163.80) -- (717.63,163.80);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (624.14,417.47) -- (717.63,417.47);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (577.40,220.17) --
	(764.37,220.17) --
	(764.37,332.91) --
	(577.40,332.91) --
	cycle;

\path[fill=fillColor] (811.11,220.17) --
	(998.08,220.17) --
	(998.08,332.91) --
	(811.11,332.91) --
	cycle;

\path[draw=drawColor,line width= 1.2pt,line join=round] (811.11,290.63) -- (998.08,290.63);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (904.60, 79.24) -- (904.60,220.17);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (904.60,445.66) -- (904.60,332.91);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (857.85, 79.24) -- (951.34, 79.24);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (857.85,445.66) -- (951.34,445.66);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (811.11,220.17) --
	(998.08,220.17) --
	(998.08,332.91) --
	(811.11,332.91) --
	cycle;
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (1084.05,597.46);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 79.24) -- ( 49.20,530.22);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 79.24) -- ( 43.20, 79.24);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,191.98) -- ( 43.20,191.98);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,304.73) -- ( 43.20,304.73);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,417.47) -- ( 43.20,417.47);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,530.22) -- ( 43.20,530.22);

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80, 79.24) {-2};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,191.98) {-1};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,304.73) {0};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,417.47) {1};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,530.22) {2};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (1084.05,597.46);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.20] at (554.02,568.72) {\bfseries Stereo(test)};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (554.02, 15.60) {Attributes};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 10.80,304.73) {Preference};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (1084.05,597.46);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 61.20) --
	(1058.85, 61.20) --
	(1058.85,548.26) --
	( 49.20,548.26) --
	cycle;

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.75] at ( 22.80,557.59) {Stereo};

\node[text=drawColor,rotate= 90.00,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.75] at ( 22.80, 18.49) {Presented Method};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (203.45, 61.20) -- (203.45, 61.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (203.45, 61.20) -- (203.45, 55.20);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (203.45, 39.60) {Preference};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (437.17, 61.20) -- (437.17, 61.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (437.17, 61.20) -- (437.17, 55.20);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (437.17, 39.60) {Immersiveness};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (670.88, 61.20) -- (670.88, 61.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (670.88, 61.20) -- (670.88, 55.20);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (670.88, 39.60) {Clarity};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (904.60, 61.20) -- (904.60, 61.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (904.60, 61.20) -- (904.60, 55.20);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (904.60, 39.60) {Naturalness};
\end{scope}
\begin{scope}
\path[clip] ( 49.20, 61.20) rectangle (1058.85,548.26);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,304.73) -- (1058.85,304.73);
\end{scope}
\end{tikzpicture}


==> SubjectiveResults_copy.tex <==
To asses the validity of the presented room equalisation approach, a  preference-based listening test has been conducted. 
\subsection[Method and Subjects]{Method and Subjects}
Ten test subjects took part in the study, all having professional or extensive personal experience with audio reproduction systems.

Subjects were asked to rate the proposed approach against several test stimuli based on the following attributes:

\noindent
\textbf{Preference:} The subjects overall subjective opinion of the presented stimuli, simply conveying which approach they would prefer to listen to given the material using.

\noindent
\textbf{Immersiveness:} Immersiveness is defined in this experiment as how psychologically connected to the audio exerts the subject feels.

\noindent
\textbf{Clarity:} For any room equalisation approach the overall goal is to improve the clarity of an reproduction system in a listening room. Subjects were asked to rate the stimuli based on both spectral and spatial clarity.

\noindent
\textbf{Naturalness:} This attribute allows the subject to rate how natural the presented stimuli would feel if the performer were imagined to be in the same room as them. Future work relating to the presented system will focus on bringing aspects of a live music venue into the listening room. Including this allows this attribute to be tracked throughout current and future iterations of the proposed method.


Subjects were asked to rate the presented stimuli on a 5 point scale with a score of 2 indicating a clear preference towards the proposed approach, 1 indicating a just noticeable preference and 0 indicating no preference to either stimuli, opposing scores indicated preference towards the test stimuli. The primary loudspeakers used for this study were Kef LS50's and Genelec 6010A Monitors for the supporting loudspeakers. These were both connected to the Max 8 test software using an RME AD-8 QS D/A converter.
\subsection[Stim]{Stimuli}

\textbf{Rear Stereo}
The original stereo material is presented both through the primary loudspeakers and the rear speakers with no alterations.

\noindent
\textbf{Front Equalisation}
The front equalisation stimulus uses the same gammatone band compensation as the proposed approach, to equalise the primary loudspeakers such that the overall transfer function matches the target function.

\noindent 
\textbf{Stereo}
Unaltered stereo playback, this being the stimulus that is is most important for the validity of the proposed method.
\subsection[Results]{Results}

Whilst the main aim of this study is to compare the proposed approach to stereo playback, a number of additional reproduction approaches have been chosen to understand in which areas the proposed approach shows improvement. The test stimuli were applied to 4 audio excerpts allowing subjects to rate each stimulus based on several genres of music. Results are shown comparing the proposed method against the following test conditions:

\noindent
 \textbf{Rear Stereo:}  Figure~\ref{RearStereoRes} shows subjects rated the test stimuli as more immersive and in some cases there appeared to be an increase in clarity. Whilst an increase in immersiveness may be expected due to the increased number of perceived sources, subjects indicated a preference towards the proposed approach showing preference towards the proposed approach is not simply due to additional loudspeakers.
    \begin{figure}
        \input{Figures/RearStereo.tex}
        \vspace{-1.8cm}
        \caption[RearStereoRes]{\footnotesize Preference study results comparing the proposed approach to the~`Rear Stereo' stimuli. A score of 2 indicates a clear preference for the proposed approach, 1 indicates a just noticeable preference towards the proposed approach and 0 indicates no preference. Opposing scores indicate a preference towards the test stimuli.}\label{RearStereoRes}
        \vspace{-0.5cm}
        \end{figure}

\noindent
\textbf{Front Equalisation:}  The results from this test stimulus (Shown in Figure~\ref{FrontEqualRes}) show a preference towards the proposed approach in all areas.
    \begin{figure}
        \input{Figures/FrontEqualisation.tex}
        \vspace{-1.8cm}
        \caption[FrontEqualRes]{\footnotesize Preference study results comparing the proposed approach to the~`Front Equalisation' stimuli.} \label{FrontEqualRes}
        \vspace{-0.5cm}
        \end{figure}

\noindent
\textbf{Stereo:} Figure~\ref{StereoRes} shows a noticeable preference towards the proposed approach for all attributes. The range of preference results, which sometimes favours stereo reproduction, may be due to subjects being used to traditional stereo playback.
    \begin{figure}
        \input{Figures/Stereo.tex}
        \vspace{-1.8cm}
        \caption[StereoRes]{\footnotesize Preference study results comparing the proposed approach to the~`Stereo' stimuli.}\label{StereoRes}
        \vspace{-0.5cm}
    \end{figure}

    \begin{figure}
        \input{Figures/MasterPlot.tex}
        \caption[Results]{All Results from pilot study}
    \end{figure}

